Study on the filters of atmospheric contamination in ground based CMB observation

The atmosphere is one of the most important contamination sources in the ground-based Cosmic Microwave Background (CMB) observations. In this paper, we study three kinds of filters, which are polynomial filter, high-pass filter, and Wiener filter, to investigate their ability for removing atmospheric noise, as well as their impact on the data analysis process through the end-to-end simulations of CMB experiment. We track their performance by analyzing the response of different components of the data, including both signals and noise. In the time domain, the calculation shows that the high-pass filter has the smallest root mean square error and can achieve high filtering efficiency, followed by the Wiener filter and polynomial filter. We then perform map-making with the filtered time ordered data (TOD) to trace the effects from filters on the map domain, and the results show that the polynomial filter gives high noise residual at low frequency, which gives rise to serious leakage to small scales in map domain during the map-making process, while the high-pass filter and Wiener filter do not have such significant leakage. Then we estimate the angular power spectra of residual noise, as well as those of the input signal for comparing the filter effects in the power spectra domain. Finally, we estimate the standard deviation of the filter corrected power spectra to compare the effects from different filters, and the results show that, at low noise level, the three filters give almost comparable standard deviations on the medium and small scales, but at high noise level, the standard deviation of the polynomial filter is significantly larger. These studies can be used for the reduction of atmospheric noise in future ground-based CMB data processing.

==> acknowledgements.tex <==
This study is supported in part by the National Key R&D Program of China No. 2020YFC2201600 and by the NSFC No.11653002.


